Compressive MRI quantification using convex spatiotemporal priors and deep auto-encoders

We propose a dictionary-matching-free pipeline for multi-parametric quantitative MRI image computing. Our approach has two stages based on compressed sensing reconstruction and deep learned quantitative inference. The reconstruction phase is convex and incorporates efficient spatiotemporal regularisations within an accelerated iterative shrinkage algorithm. This minimises the under-sampling (aliasing) artefacts from aggressively short scan times. The learned quantitative inference phase is purely trained on physical simulations (Bloch equations) that are flexible for producing rich training samples. We propose a deep and compact auto-encoder network with residual blocks in order to embed Bloch manifold projections through multiscale piecewise affine approximations, and to replace the nonscalable dictionary-matching baseline. Tested on a number of datasets we demonstrate effectiveness of the proposed scheme for recovering accurate and consistent quantitative information from novel and aggressively subsampled 2D/3D quantitative MRI acquisition protocols.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> sections/partitioning.tex <==
\subsection{Parameter inference using deep auto-encoder}
%After reconstructing the compressed principal TSMI and reducing strong aliasing artefacts in them, it is time to estimate the underlying parametric maps. This is done by processing the per-voxel temporal (magnetisation) signal trajectories and fit them to the physical model driven by the Bloch equations. The baseline MRF approach exhaustively simulates a large dictionary of magnetic responses (fingerprints) for all combinations of the quantised NMR parameters. The MRF dictionary discretises (densely samples) the low-dimensional manifold of Bloch equation solutions. The task of fitting or projecting to this non-linear manifold, is then approximated by nearest neighbour searches (NNS)  to identify the most correlated fingerprint and its corresponding NMR parameters for each (normalised) voxel of the principal TSMI $\widehat X$:
%\eql{
%	[\Theta_v] = \text{NNS}_{D}(\widehat X_v), \quad \forall v=1,\hdots,n.}
%Here $\text{NNS}_D(x):=\argmin_j\norm{x-D_j}_2$ denotes the nearest neighbour search %\footnote{Back-projected voxels and dictionary atoms $\{X_v\}, \{D\}_j$ are both normalized before fed into NNS.} 
%which serves as a Euclidean projection onto the discrete set of fingerprints i.e. the manifold of Bloch equation solutions.  
%%As occurs to any multi-parametric manifold enumeration, the main drawback of such approach is the size of  this dictionary which grows exponentially in terms of the number of parameters and their quantization resolution;  a serious (non-scalability) limitation of the current methods to be applicable in the emerging multi-parametric MRF applications
%However, enumerating the multi-parametric MRF manifold in order for~\eqref{eq:NNS} to be an accurate projection introduces an exponentially growing complexity (in terms of $P$) to the storage and computations needed for conducting NNS. %(i.e. performing an exact search on a huge dictionary). 
%\todo{A number of approaches e.g. \nref cauley, to accelerate the NNS step in DM, the essence of which is to partition/group the fingerprints into hiearchies e.g. trees.}
%A recent line of research~\cite{CoverBLIP-MLSP, inexactipg-tit} shows that certain tree search strategies can benefit from 
%the low \emph{intrinsic dimensionality} of the MRF manifold and significantly accelerate the matching step. 
%%and facilitate fast searches with \emph{sub-linear} complexities in $d$. 
%However storage of the dictionary or the corresponding tree still remains a big challenge for fine-grid enumerations.

\subsubsection{Encoder}
%\eql{\Theta_v = \Ff(\widehat X_v), }
%where, $\widehat X_v$ denotes the normalised/standardised temporal signal $X_v$ at each voxel $v$, and $\Ff(x) \approx \argmin_{\Theta} \norm{x-\Bb(\Theta)}_2$ for input signals $x$ in a neighbourhood of $\Bb$.

Instead of using a large-size dictionary for DM, we propose training and using a compact deep residual network coined as MRFResnet to regress the NMR parameters in a computably efficient manner. 
This network learns to approximate Bloch manifold projections through a continuous mapping  $\Rr: \widehat X_v \rightarrow\Theta_v$ parametrised by the network's weights and biases $\{W,\beta\}$:
\begin{align}
\Rr(x) \equiv h^{(N+1)}(x)=\phi\left(W^{(N+1)}h^{(N)}(x)+\beta^{(N+1)}\right) \label{eq:resnet1}
\end{align}
where $h^{(i)}$ the outputs of $i=1,\ldots,N$ residual blocks are
\begin{align*}
&h^{(i)}(x)= \phi\left( h^{(i-1)}(x) + g^{(i)}(x)  \right), \\
&g^{(i)} (x)= W^{(i,2)}\phi\left(W^{(i,1)}h^{(i-1)}(x)+\beta^{(i,1)}\right)+\beta^{(i,2)},
\end{align*}
$h^{(0)}(x)=x$ and the ReLU activations $\phi(x)=\max(x,0)$ are used throughout.
 The inputs to the MRFResnet are the normalised temporal voxels of the principal TSMI. The network is trained on simulated noisy Bloch responses (see section~\ref{sec:algosetup}) so that the approximate projection holds
 %$\Rr(x) \approx \argmin_{\Theta} \norm{x-V^H\Bb(\Theta)}_2$ 
 \eql{ \Rr(x) \approx \Pp_\Bb(x)
 }
 in a neighbourhood of the (compressed) Bloch manifold.

 \subsubsection{Decoder}
The proton density (PD) is a scaling factor that amplifies the Bloch responses in each voxel. Hence after estimating other nonlinear NMR parameters (e.g. T1/T2) using MRFResnet, PD can be explicitly resolved through~\eqref{eq:PDestim}. 
%\nref [blip, coverblip]: 
%\begin{align} 
%\gamma_v= \frac{\langle VX_v, \Bb(\Theta_v)\rangle}{\norm{\Bb(\Theta_v)}^2} \approx \frac{\langle X_v, V^H\Bb(\Theta_v)\rangle}{\norm{V^H\Bb(\Theta_v)}^2}.
%\end{align} 
This would however require evaluating/solving Bloch responses for all voxels and their parameters $\Theta_v$ which can be computationally intensive. Instead we train a \emph{decoder} network $\Gg(.)$ which for given NMR parameters 
%$\Gg: \Theta_v \rightarrow V^H\Bb(\Theta_v)$ 
\eql{\Gg(\Theta_v) \approx V^H\Bb(\Theta_v)
}
it approximately generates the corresponding compressed Bloch responses (clean fingerprints) in short runtimes. 
For the acquisition sequence in our experiments, it turns out that a fully-connected shallow network with one hidden layer and ReLU activations can approximate well this step.\footnote{We also observed a similar network complexity for generating responses to the well-known FISP sequence~\cite{FISP}. However, we did not achieved accurate predictions using shallow architectures of comparable sizes for $\Rr$ (two layer were needed at least however with larger model than MRFResnet)~\cite{deepMRFgeom, LRTVismrm}. This suggests that generating clean responses was easier than projecting noisy fingerprints back to their generative parameters (inverse), and the latter requires deep processing (see section~\ref{sec:partitioninig}).
} 
%i.e. $\Gg(x)\equiv W'^{(2)}\phi\left(W'^{(1)}x+\beta'^{(1)}\right)+\beta'^{(2)}$.


Subspace compression helps reducing model sizes in both networks (hence the risk of overfitted predictions) and also reducing required training resources compared to uncompressed deep MRF approaches e.g.~\cite{DRONE-MRF,betterreal}. Further to avoid loosing discrimination between fingerprints \textemdash e.g. by a magnitude-only data processing~\cite{DRONE-MRF} \textemdash we adopt a practical phase-alignment heuristic from~\cite{coverblip_iop,AIRMRF} 
%which assumes principal magnetisation responses having constant complex phases across temporal domain, 
%which uses per-voxel complex angles corresponding to the first principal component i.e. $V^H_{s=1}\widehat X, V^H_{s=1}D$, 
to de-phase TSMIs and training samples before being fed to the MRFResnet. This treatment allows both networks with loosing generality have real-valued parameters and approximate real-valued mappings.\footnote{Another way is to duplicate input size by separating real and imaginary signal components e.g.~\cite{betterreal}). We found this unnecessary in our experiments.}
%With this treatment we can assume without loss of generality both networks have real-valued parameters and approximate real-valued mappings.\footnote{Another common way (see e.g.~\cite{betterreal}) is to duplicate the inputs size by separating the real and imaginary signal components, however we found that unnecessary in our experiments.}

%====================================
\begin{figure}[t!]
	\centering
	\begin{minipage}{\linewidth}
		\centering
		\includegraphics[trim=10 40 0 100,clip,width=\linewidth]{../gen_figs/NET.pdf} 	
		\caption{\footnotesize{MRFResnet $\Rr$ (encoder), the Bloch response generative network $\Gg$ (decoder), and the \emph{implicit} linear dimensionality reduction/expansion (first/last) layers using the subspace model $V^H/V$. 
		} \label{fig:net}}
	\end{minipage}
\end{figure}
%=====================================	
Figure~\ref{fig:net} shows the MRFResnet and generative networks cascaded to each other. Unit dimensions are customised to an MRF sequence used in our experiments encoding T1/T2 relaxation times, with reduced subspace dimension $s=10$.   
 %The corresponding Bloch responses 
%samples (i.e. dictionary fingerprints) corresponding to this sequence
 %live in a low-rank subspace of dimension $s=10$ which determines $\Rr$'s input and $\Gg$'s output dimensions.  
 MRFResnet has $N=6$ residual blocks 
 %each having a skip connection bypassing two fully connected layers 
 of 10 neurons width, whereas $\Gg$ has one hidden layer with 300 neurons. 
Cascading both networks resembles the topology of \emph{auto-encoders}~\cite{SDAE_bengio}. Auto-encoders are proven powerful in denoising tasks through creating an \emph{information bottleneck} which corresponds to learning/using a low-dimensional manifold model for capturing (nonlinear) intrinsic signal structures. 
%, and then projecting noisy data samples onto this model.
%projecting noisy data on the low-dimensional manifold models representing the (nonlinear)  intrinsic structures of data. 
In our task computed TSMI voxels are processed by a similar architecture to create clean magnetisation responses as well as estimating the intrinsic NMR parameters. The $p=2$ neurons bottleneck here has a physical interpretation: fitting noisy temporal trajectories to the nonlinear Bloch model with limited $p\ll T$ degrees of freedom determined by the T1/T2 quantities.
%projecting onto the manifold of Bloch responses whose intrinsic dimension is $p\ll L$ the number of NMR parameters.


%
%Considering the (implicit) subspace projection and lifting ($V^H,V$) on its both ends, the input/output temporal signals despite their high ambient dimensions  dimension is reduced to  
%
%By considering the subspace projection and lifting as two linear layers that implicitly appearing on both ends, we have a network that manifest an auto-encoder topology \nref. 
%%This approximation would be valid for a small enough neighbourhood of the manifold i.e. signals with moderate perturbations i.e. 
%Figure \nref illustrates the MRFResnet. Dimensions of the input/output and hidden units are customised here for the \todo{name\nref}sequence which encodes $p=2$ NMR characteristics i.e. the $\Theta=\{$T1, T2$\}$ relaxation times. 
% (the original temporal dimension was $L=880$ where after the SVD compression is reduced to $S=10$, hence the input dimension). Training samples (i.e. MRF dictionary) corresponding to the \todo{name} sequence despite their high ambient dimension $L=880$ live in a low-rank subspace and are well represented by very few  principal components~\cite{SVDMRF} e.g. $s=10$ here, which determines first layer's dimension accordingly. 
% Each residual block  consists of a skip connection bypassing two fully connected layers with 10 neurons each. 
% This is equivalent to using a 10-channel $1\times1$ spatial (convolution) filter at each layer since at this stage we do temporal processing at each voxel separately. 


%We use Adam algorithm~\nref to optimize~\eqref{eq:reg}  where the gradient updates 
%are computed by the standard back-propagation algorithm.

%For further robustness, the on-the-fly noise level (40 dB) are added to the training data. Note we update the noise at the beginning of each training epoch, i.e., before the computation moving to feedforward phase.



\section{Hierarchical partitioning of the Bloch response manifold}
\label{sec:partitioninig}
In this part we show that the MRFResnet provides a multi-scale piecewise affine approximation to the Bloch response manifold projection \eqref{eq:proj}. 
Hierarchical partitioning and multi-scale approximations are also central to fast search schemes proposed for the DM-based MRF (see illustrations in \cite{coverblip_iop,CoverBLIP-MLSP})
%for multilevel Bloch manifold partitions resulted by adopting a cover tree search strategy). 
However unlike any form of DM (fast or exhaustive) that creates point-wise approximations for 
%for the manifold projection 
\eqref{eq:NNS}, 
MRFResnet does not memorise a dictionary and rather use it to learn and efficiently encode a compact set of partitions and \emph{deep matched-filters} for affine regression of the NMR quantities.
%In this part we show that the MRFResnet provides a multi-scale piecewise affine approximation to the Bloch response manifold projection \eqref{eq:proj}. This would imply partitioning the manifold into a number of clusters at each scale and approximate per-cluster projections by an affine operator i.e. projection on a flat surface approximating that partition (a similar idea has been deliberately crafted and illustrated in GMRA \nref without using deep neural networks and gradient-based learning). We illustrate that by progressing into deeper residual blocks the input space partitions become finer implying a tighter level of approximations at lower (deeper) scales. Hierarchical partitioning and multi-scale approximations are similarly central to the fast search schemes proposed for the DM-based MRF (see illustrations in \nref [coverblip] for multilevel Bloch manifold partitions resulted by adopting a cover tree search strategy). 
%However unlike any form of DM (fast or exhaustive) that creates point-wise approximations for the manifold projection \nref(Eq), MRFResnet does not memorise a MRF dictionary but rather use it to learn and encodes a compact set of partitions and \emph{deep matched-filters} for affine regression of the NMR quantities in each segment.




\subsection{Affine spline function approximation}
Networks such as MRFResnet (also the decoder $\Gg$) composed of piecewise linear activation functions e.g. ReLU and the (linear) identity activations used in skip connections 
%we have that (see e.g.~\cite{splineDN, montufar2014number}): each layer's output is a piece-wise affine transformation of its direct input. Composition of such layers 
result in piecewise affine functions $h^{(i)}(x)$ after each residual block as well as the end-to-end mapping $\Rr(x)$~(see e.g.~\cite{splineDN, montufar2014number}). Further $\Rr$ is \emph{Lipschitz continuous} for continuous activation functions (as above) and for bounded $\{W^{(i)}, \beta^{(i)}, i\}$. %\nref[cite]

%Considering the prediction of $\Rr$ (before last ReLU layer which imposes positive T1/T2 values)
%\eql{z^{(N)} (x):= W^{(N)} h^{(N-1)}+\beta^{(N)} }

%Therefore we simply refer to $z^{(N)} (x)$ as "output" in our analysis.
{\thm{
Denote by $z:\RR^s \rightarrow \RR^p$
\eql{ z(x):= W^{(N+1)} h^{(N) }(x)+\beta^{(N+1)} }
the \emph{weighted outputs} in \eqref{eq:resnet1} before the last non-linearity.\footnote{The last ReLU layer in $\Rr$ is for imposing the positivity of T1/T2 values, and therefore the prediction task is mainly done by the preceding layers. } The following \underline{affine spline representation} holds for MRFResnet:
\eql{ z(x) = \A[x]x+\b[x] :=\sum_r \left( A_r x+b_r \right)\iota_{\Omega_r}(x), \label{eq:spline}}
where $\iota_{\Omega_r}(x)$ is the indicator function with respect to a segment (set) $\Omega_r\in \RR^s$, returning $x$ if it belongs to the segment and 0 otherwise \textemdash segments form a disjoint partitioning of the input space with affine boundaries. Matrices $A_r\in\RR^{p\times L}$ and vectors $b_r\in\RR^p$ define the corresponding slopes and offsets for the input-output affine mapping in each segment. Shorthands $\A[x]: \RR^s\rightarrow \RR^p$ and $\b[x]:\RR^s\rightarrow \RR^p$ represent the input-dependent (piece-wise affine) mapping of $z(x)$. $\b[x]$ represents $p$ input-dependent offsets. Similarly, $\A[x]$ is an input-dependent $p\times s$ matrix where each row is a \underline{deep matched-filter} returning its correlation with $x$ for each output. }}

Proof can be found in~\cite{splineDN} for general feedforward networks with fully-connected, convolutional, pooling and/or residual layers and using any piecewise-linear activations. 
%Matched-filters and offsets here are used for \emph{regressing} the outputs \textemdash not to be confused with the MRF dictionary matching (DM). % in baseline MRF reconstruction.
% In other word, d
During training MRFResnet learns $\{W^{(i)}, \beta^{(i)}\}$ or equivalently $\{\A[x],\b[x]\}$ to provide a continuous and piece-wise affine \emph{approximation} for~\eqref{eq:proj}. 
%between input and outputs e.g. the Bloch manifold projection \nref(eq) for the MRF problem. 
The universal approximation theorem~\cite{cybenko1989} states that a shallow network with one but very wide hidden layer can do this.
 %provide an arbitrarily close approximation to any Borel-measurable function. 
 Deeper networks are however more practical to efficiently reduce the number of hidden units~\cite{shallowdeep-bengio}. Indeed, we experimentally observe this (section~\ref{sec:deepvskm}) by comparing MRFResnet to a shallow learning scheme related to~\cite{PERK} based on Kernel Machines (KM) and random features~\cite{fastfood}. 
 %\todo{also say this is better than MRFNET, drone, .. because its deeper}
 %For certain manifold embedding tasks this has been proven e.g. in~\cite{deepmanifold-basri,coifman-manifoldDN,geometricDL,dongdong_manifold}. 

%%============
\begin{figure*}[t!]
	\centering
	\scalebox{1}{
	\begin{minipage}{\linewidth}
		\centering		
		\includegraphics[trim=115 25 110 75,clip, width=.165\linewidth]{../gen_figs/figs4/segments/manif_seg_1.png}\hspace{-.1cm}
		\includegraphics[trim=115 25 110 75,clip,width=.165\linewidth]{../gen_figs/figs4/segments/manif_seg_2.png}\hspace{-.1cm}
		\includegraphics[trim=115 25 110 75,clip,width=.165\linewidth]{../gen_figs/figs4/segments/manif_seg_3.png}\hspace{-.1cm}
		\includegraphics[trim=115 25 110 75,clip,width=.165\linewidth]{../gen_figs/figs4/segments/manif_seg_4.png}\hspace{-.1cm}
		\includegraphics[trim=115 25 110 75,clip,width=.165\linewidth]{../gen_figs/figs4/segments/manif_seg_5.png}\hspace{-.1cm}
		\includegraphics[trim=115 25 110 75,clip,width=.165\linewidth]{../gen_figs/figs4/segments/manif_seg_6.png}
		\\
		\includegraphics[width=.165\linewidth]{../gen_figs/figs4/segments/seg_1.pdf}\hspace{-.1cm}
		\includegraphics[width=.165\linewidth]{../gen_figs/figs4/segments/seg_2.pdf}\hspace{-.1cm}
		\includegraphics[width=.165\linewidth]{../gen_figs/figs4/segments/seg_3.pdf}\hspace{-.1cm}
		\includegraphics[width=.165\linewidth]{../gen_figs/figs4/segments/seg_4.pdf}\hspace{-.1cm}
		\includegraphics[width=.165\linewidth]{../gen_figs/figs4/segments/seg_5.pdf}\hspace{-.1cm}
		\includegraphics[width=.165\linewidth]{../gen_figs/figs4/segments/seg_6.pdf}	
\caption{\footnotesize{Coarse-to-fine partitioning of the Bloch manifold (top row) sampled by a dense fingerprinting dictionary (3D visualisations used PCA), and their generative T1/T2 parameters (bottom row) using MRFResnet. From left to right figures illustrate learned partitions after each residual block. }
%The space dimension in (a) is $s=10$ but visualised across 3 dimensions using PCA.
\label{fig:seg}}
\end{minipage}}
\end{figure*}
%============

%=====================
\begin{figure}[t!]
	\centering
	\scalebox{1}{
	\begin{minipage}{\linewidth}
		\centering		
		\subfloat[The average magnetic response]{
		\includegraphics[width=.485\linewidth]{../gen_figs/figs4/segments/avg_signal.pdf}}\hspace{-.1cm}
		\subfloat[Centred magnetic responses]{
		\includegraphics[width=.485\linewidth]{../gen_figs/figs4/segments/difference_signal.pdf}}\\
		\subfloat[T1 deep matched filter]{
		\includegraphics[width=.485\linewidth]{../gen_figs/figs4/segments/T1_filter.pdf}}\hspace{-.1cm}	
		\subfloat[T2 deep matched filter]{
		\includegraphics[width=.485\linewidth]{../gen_figs/figs4/segments/T2_filter.pdf}}	
\caption{ \footnotesize{(a) The mean and (b) the centred magnetic responses i.e. fingerprints within the range (T1, T2) $\in [1000-1200]\times[80-110]$ (ms). (c)-(d) The end-to-end match filters learned by the MRFResnet to regress T1/T2 values shown across the original (non-compressed) temporal dimension.} \label{fig:matchfilt}}
\end{minipage}}
\end{figure}
%============


\subsection{Visualising MRFResnet segments on Bloch manifold}

{\rem{\emph{Continuity of $z(x)$ implies that adjacent segments $\Omega_r,\Omega_{r'}$  correspond to distinct $A_r,A_{r'}$. 
Indeed, if $A_r=A_{r'}$ and the only difference is in the offsets $b_r\neq b_{r'}$, then $\Omega_r,\Omega_{r'}$ won't intersect on boundaries. Therefore they are not adjacent segments unless contradicting the continuity assumption.}}}

This remark gives an idea for visualizing the input space segments.  
For densely sampled input signals $x$, we compute derivatives of the weighted outputs with respect to inputs using \emph{back propagation}. These will determine the input-dependant slopes in the affine spline formulation \eqref{eq:spline} i.e. rows of $\A[x]$ at a point $x$ are populated as follows $\forall j=1,2,\ldots,p$:%\footnote{For a matrix $X$ we denote by $X_{(p,.)}$ as its $p$-th row. For a vector $x$, $x_p$ denotes its $p$-th element. We also later denote by $\mathbf{e}_p$ the coordinate vector whose $p$-th element is one and zero elsewhere.}  
\begin{align}
	\A[x]_{(j,.)}%&=\left(\nabla_x z^{(N)}_{p}(x)\right)^T \nonumber\\  %\frac{\partial z^{(N)}_{p}(x)}{\partial x}:=\\
	=\left[ \frac{\partial z_{j}(x)}{\partial x_1}, \frac{\partial z_{j}(x)}{\partial x_2},\ldots,\frac{\partial z_{j}(x)}{\partial x_s} \right]. \label{eq:grad}
\end{align} 
%For a given input $x$ the gradients in \eqref{eq:grad} 
%which can be efficiently calculated using \emph{back-propagation}. 
%We feed forward $x$ to identify all activations $z^{(i)},h^{(i)}$ and then follow the recursion starting at the vector $y = \mathbf{e}_p$: %\footnote{$\mathbf{e}_p$ the coordinate vector whose $p$-th element is one and zero elsewhere}
%\begin{align} 
%%&y = \mathbf{e}_p	\\
%&y \leftarrow f_i'(z^{(i-1)}) \odot \left( \left(W^{(i)}\right)^Ty\right) \quad i=N,N-1,\ldots,2.\nonumber\\
%&\nabla_x z^{(N)}_{p}(x) = \left(W^{(1)}\right)^Ty,
%\end{align}
%%where $\mathbf{e}_p\in \RR^L$ is the coordinate vector whose $p$-th element is one and zero elsewhere, and 
%where $\odot$ denotes  the element-wise vector product, and $f_i'(.)$ denotes the (element-wise) derivative of the activation function. For an identity activation $f_i'(.)$ is an all-one vector and for the ReLU activation it returns one for the positive (direct) input coordinates and zero elsewhere. 
By vector quantisation (e.g. k-means clustering) we cluster regions of $x$ that output distinct slopes $A_r$  and identify the segments $\Omega_r$. Similar routine could apply to compute input space partitions by clustering back-propagated output derivates after each residual block (Theorem 1 and Remark 1 also hold for the intermediate blocks of $\Rr$). 

According to~\cite{splineDN} as we progress into deeper layers partitions will be sub-dived into smaller segments in a \emph{hierarchal} fashion. This can be observed in Figure~\ref{fig:seg} where we adopted the above routine for a T1/T2 encoding MRF sequence used in our experiments and visualise multi-scale (from coarse-to-fine) partitions obtained after each residual layer. %as well as the final layer of the MRFResnet. % for a Bloch response manifold (used in our 2D MRF acquisition sequence, see section\nref).
%We note that for a classification problem~\cite{splineDN} used a similar idea to separately identify each hidden layer's segments and then intersect them in a hierarchical (layer-by-layer) fashion to get $\Omega_r$.
%Due to the fine sampling of the input space this approach is not computational/memory friendly, however, it 
The Bloch response manifold is sampled across fine-gridded T1/T2 values (i.e. MRF dictionary) to visualise the intersection of the input space segments with this manifold (results are visualised across the three dominant principal component axes). 
MRFResnet learns about a thousand partitions for the end-to-end mapping $z(x)$. In the light of~\eqref{eq:spline} we know that for each partition $\Omega_r$ the network implicitly encodes $p=2$ deep matched-filters (the rows of $\A[x]$ or alternatively $A_r$) and an offset term to linearly regress the T1/T2 outputs in that segment. As such  instead of memorising $>$100K dictionary atoms used for training, the network learns a compact piece-wise affine approximation to the Bloch manifold projection~\eqref{eq:proj} as a rapid and memory-efficient alternative to DM's point-wise approximation~\eqref{eq:NNS} for NMR parameter inference.
% than DM (which implements inefficient point-wise manifold approximations for \nref(Eq) for this task). 
%which is computationally and memory-wise
Figure~\ref{fig:matchfilt} shows the magnetic responses 
%(the mean and centred fingerprints) 
for a range of T1/T2 values, as well as deep matched-filters learned by MRFResnet to predict each of these quantities in this range from noisy inputs. 
Computed trough \eqref{eq:grad}, match-filters are one-dimensional analogues of the \emph{saliency maps} a.k.a. \emph{deep dream images}~\cite{saliency}, measuring sensitivities of the neurons with respect to the inputs. 
%As can be seen in Figure~\nref, matched-filters peak at discriminant parts of the fingerprints that  is where the sequence encodes a significant amount of information about the underlying NMR characteristics\todo{keep-or-dlt}.

%\begin{figure}
%	\centering
%	\scalebox{1}{
%	\begin{minipage}{\linewidth}
%		\centering		
%		\includegraphics[trim=115 25 110 75,clip, width=.33\linewidth]{../gen_figs/figs4/segments/manif_seg_1.png}\hspace{-.1cm}
%		\includegraphics[trim=115 25 110 75,clip,width=.33\linewidth]{../gen_figs/figs4/segments/manif_seg_2.png}\hspace{-.1cm}
%		\includegraphics[trim=115 25 110 75,clip,width=.33\linewidth]{../gen_figs/figs4/segments/manif_seg_3.png}\\
%		\includegraphics[trim=115 25 110 75,clip,width=.33\linewidth]{../gen_figs/figs4/segments/manif_seg_4.png}\hspace{-.1cm}
%		\includegraphics[trim=115 25 110 75,clip,width=.33\linewidth]{../gen_figs/figs4/segments/manif_seg_5.png}\hspace{-.1cm}
%		\includegraphics[trim=115 25 110 75,clip,width=.33\linewidth]{../gen_figs/figs4/segments/manif_seg_6.png}
%		\\
%		\includegraphics[width=.33\linewidth]{../gen_figs/figs4/segments/seg_1.pdf}\hspace{-.1cm}
%		\includegraphics[width=.33\linewidth]{../gen_figs/figs4/segments/seg_2.pdf}\hspace{-.1cm}
%		\includegraphics[width=.33\linewidth]{../gen_figs/figs4/segments/seg_3.pdf}\\
%		\includegraphics[width=.33\linewidth]{../gen_figs/figs4/segments/seg_4.pdf}\hspace{-.1cm}
%		\includegraphics[width=.33\linewidth]{../gen_figs/figs4/segments/seg_5.pdf}\hspace{-.1cm}
%		\includegraphics[width=.33\linewidth]{../gen_figs/figs4/segments/seg_6.pdf}	
%\caption{\footnotesize{Coarse-to-fine partitioning of (a) the Bloch manifold sampled by a dense fingerprinting dictionary (3D visualisation used PCA), and (b) their generative T1/T2 parameters, learned by the MRFResnet. From left to right, top rows in (a) and (b) illustrate the partitions after residual blocks 1 to 3 (similarly 4 to 6 in the bottom rows). }
%%The space dimension in (a) is $s=10$ but visualised across 3 dimensions using PCA.
%\label{fig:seg}}
%\end{minipage}}
%\end{figure}


